UI-Venus-1.5 Technical Report

GUI agents have emerged as a powerful paradigm for automating interactions in digital environments, yet achieving both broad generality and consistently strong task performance remains challenging. In this report, we present UI-Venus-1.5, a unified, end-to-end GUI Agent designed for robust real-world applications. The proposed model family comprises two dense variants (2B and 8B) and one mixture-of-experts variant (30B-A3B) to meet various downstream application scenarios. Compared to our previous version, UI-Venus-1.5 introduces three key technical advances: (1) a comprehensive Mid-Training stage leveraging 10 billion tokens across 30+ datasets to establish foundational GUI semantics; (2) Online Reinforcement Learning with full-trajectory rollouts, aligning training objectives with long-horizon, dynamic navigation in large-scale environments; and (3) a single unified GUI Agent constructed via Model Merging, which synthesizes domain-specific models (grounding, web, and mobile) into one cohesive checkpoint. Extensive evaluations demonstrate that UI-Venus-1.5 establishes new state-of-the-art performance on benchmarks such as ScreenSpot-Pro (69.6%), VenusBench-GD (75.0%), and AndroidWorld (77.6%), significantly outperforming previous strong baselines. In addition, UI-Venus-1.5 demonstrates robust navigation capabilities across a variety of Chinese mobile apps, effectively executing user instructions in real-world scenarios. Code: https://github.com/inclusionAI/UI-Venus; Model: https://huggingface.co/collections/inclusionAI/ui-venus

==> doc/data.tex <==
\section{Data Construction}

\subsection{Data Overall}


\noindent \textbf{Grounding:} Our training data contains approximately 100K open-source GUI grounding instances (Table. \ref{groundingdata}) sampled from Widget Captioning~\citep{cheng2024seeclickharnessingguigrounding}, UI RefExp~\citep{bai2021uibertlearninggenericmultimodal}, ShowUI web~\citep{lin2024showuivisionlanguageactionmodelgui}, and OmniAct~\citep{kapoor2024omniactdatasetbenchmarkenabling}, which are extracted from different platforms such as mobile, desktop, and web. 


\input{tables/gd_data}


\noindent \textbf{Navigation:} we first collect rich open-source dataset like 

\input{tables/navi_data}



\subsection{Action Space}

Following UI-TARS\citep{} and Qwen2.5VL\citep{}, we define a new action space which is more compatible with the existing open-source navigation training data. 




\subsection{Data Cleaning}

\noindent \textbf{Grounding:}

\noindent \textbf{Navigation:} 



trace score

data annotation

==> tables/androidlab_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Gemini-1.5-Pro~\citep{team2024gemini}                      &  -    & 16.7                           \\ 
    GLM4-9B-ft~\citep{glm2024chatglm}                      &  9B    &  21.0                        \\ 
    LLaMA3.1-ft~\citep{grattafiori2024llama}                      &  8B    & 23.9                         \\ 
    GPT-4o~\citep{hurst2024gpt}       &   -        & 31.2  \\
    Qwen3-VL-2B\textsuperscript{*}~\citep{Qwen3-VL}   &  2B    & 33.3                           \\ 
    Qwen3-VL-8B\textsuperscript{*}~\citep{Qwen3-VL}  &  8B    &       43.5                  \\ 
    Qwen3-VL-30B-A3B\textsuperscript{*}~\citep{Qwen3-VL}  &  30B &      42.0                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
    AutoGLM~\citep{liu2024autoglm}       & -        & 36.2  \\
    V-Droid~\citep{dai2025advancing}  & 8B   & 38.3           \\
    UI-Genie~\citep{xiao2025ui} & 72B & 41.2  \\
    MobileUse~\citep{li2025mobileuse}  & 72B   & 44.2    \\
    UI-Venus-1.0-7B~\citep{gu2025ui} & 7B   &   41.3  \\
    UI-Venus-1.0-72B~\citep{gu2025ui} & 72B   &  49.3   \\
    AutoGLM-Mobile~\citep{liu2024autoglm}  & 9B   & 46.8    \\
    AutoGLM-Phone-9B-Multilingual~\citep{liu2024autoglm}  & 9B   & 47.7    \\
    Step-GUI-4B\textsuperscript{*}~\citep{yan2025step}  &  4B     &  47.8              \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &             \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{AndroidLab} for end-to-end models. \textsuperscript{*} indicates that the results were evaluated by us. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:AndroidLab}
\end{table}


==> tables/cagui_exp.tex <==
\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lccc}
    \toprule
    \textbf{Models} & \textbf{Fun2Point} & \textbf{Text2Point}    & \textbf{Avg}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Closed-source Models}} \\
    GPT-4o~\citep{openai2024gpt4o}                           & 22.1          & 19.9                 &            21.0             \\ 
    GPT-4o w grounding~\citep{openai2024gpt4o}                           & 44.3          & 44.0                 &   44.2    \\        
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Open-source Models}} \\
    Intern2.5-VL-8B~\citep{chen2024expanding}                      & 17.2          & 24.2                          &     20.7        \\ 
    Intern2.5-VL-26B~\citep{chen2024expanding}                      & 14.8          & 16.6                        &        15.7      \\ 
    Qwen2.5-VL-7B~\citep{bai2025qwen25vltechnicalreport}                      & 59.8          & 59.3                &   59.6                     \\ 
    OS-Genesis-7B~\citep{osgenesis}                        & 8.3          & 5.8                 &   7.1    \\
    OS-Atlas-7B~\citep{wu2024osatlasfoundationactionmodel}                 & 53.6          & 60.7                 &   57.2           \\
    Aguvis-7B~\citep{xu2024aguvis}                        & 60.8          & 76.5                 &                68.7         \\
    UI-TARS-7B~\citep{qin2025uitarspioneeringautomatedgui}                        & 56.8          & 66.7                 &         61.8                 \\
    AgentCPM-GUI~\citep{agentcpm}                        & 79.1&76.5                &        77.8                \\
    \midrule
    \rowcolor{gray!15}
    \multicolumn{4}{l}{\textit{Ours}} \\
    UI-Venus-Ground-7B                        & { \ul 83.3} &  { \ul 83.2} & { \ul 83.3}         \\ 
    UI-Venus-Ground-72B                        & \textbf{84.1} & \textbf{85.9}        & \textbf{85.0}               \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{CA-GUI} grounding dataset. Our UI-Venus-72B achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:AgentCPM-GUI}
\end{table}


==> tables/gd_data.tex <==
% \begin{table*}[h]
% \centering
% \begin{tabular}{c|ccccc|c}
% \toprule
%                       & \textbf{widge\_captioning} & \textbf{UI\_refexp} & \textbf{Seeclick} & \textbf{ShowUI} & \textbf{Omniact} & \textbf{Total} \\ \hline
% \textbf{\#Samples} & 32742                      & 13084               & 38146             & 19435           & 3721             & 107128         \\ \bottomrule
% \end{tabular}
% \label{groundingdata}
% \caption{Basic statistics for grounding training data from different datasets.}
% \end{table*}



% \begin{table}[h]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{8pt}
% \begin{tabular}{l c}
% \toprule
% \textbf{Dataset} & \textbf{\# Samples} \\
% \midrule
% Widget Captioning & 32,742 \\
% UI RefExp & 13,084 \\
% SeeClick & 38,146 \\
% ShowUI & 19,435 \\
% OmniAct & 3,721 \\
% \midrule
% \textbf{Total} & \textbf{107,128} \\
% \bottomrule
% \end{tabular}
% \vspace{0.3em}
% \caption{Training data composition for GUI grounding tasks across different datasets.}
% \label{tab:grounding_data}
% \end{table} 

% \begin{table*}[h]
% \centering
% \footnotesize
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{c*{6}{c}} 
% \toprule
% \textbf{} & \textbf{Widget Captioning} & \textbf{UI RefExp} & \textbf{SeeClick} & \textbf{ShowUI} & \textbf{OmniAct} & \textbf{Total} \\
% \midrule
% \textbf{\# Samples} & 32,742 & 13,084 & 38,146 & 19,435 & 3,721 & \textbf{107,128} \\
% \bottomrule
% \end{tabular}
% \vspace{0.4em}
% \caption{Training data composition for GUI grounding tasks. Our training dataset comprises 107K samples from five complementary sources.}
% \label{tab:grounding_data}
% \end{table*}



\begin{table*}[h]\small
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|ccccc|c}
\toprule
\textbf{} & \textbf{Widget Captioning} & \textbf{UI RefExp} & \textbf{SeeClick-Web} & \textbf{ShowUI} & \textbf{OmniAct} & \textbf{Sampled training set} \\
\midrule
\textbf{\# Samples} & 34k & 17k & 325k & 110k & 141k  & \textbf{107k} \\
\bottomrule
\end{tabular}
\vspace{0.4em}
\caption{GUI grounding data composition. Our training dataset comprises 107k samples from five complementary sources.}
\label{tab:grounding_data}
\end{table*}

==> tables/navi_data.tex <==
% \begin{table*}[h]
% \centering
% \begin{tabular}{c|ccccccc|cc}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}}           & \multicolumn{7}{c|}{\textbf{Multiple Steps}}                                                                                                                                                                         & \multicolumn{2}{c}{\textbf{Single Step}}          \\ 
%  & \multicolumn{1}{c}{\textbf{GUI-O}} & \multicolumn{1}{c}{\textbf{AITZ}} & \multicolumn{1}{c}{\textbf{AC}} & \multicolumn{1}{c}{\textbf{Aitw}}  & \multicolumn{1}{c}{\textbf{Amex}}  & \multicolumn{1}{c}{\textbf{CN-Navi*}} & \textbf{Total}  & \multicolumn{1}{c}{\textbf{GD*}} & \textbf{VQA*} \\ \hline
% \textbf{\#Samples}     & \multicolumn{1}{c}{114130}      & \multicolumn{1}{c}{13426}  & \multicolumn{1}{c}{84189}           & \multicolumn{1}{c}{35018} & \multicolumn{1}{c}{40153} & \multicolumn{1}{c|}{11037}       & 222183 & \multicolumn{1}{c}{107128}     & 41936   \\ \
% \textbf{\#Traces}    & \multicolumn{1}{c}{7406}        & \multicolumn{1}{c}{2099}   & \multicolumn{1}{c}{13353}           & \multicolumn{1}{c}{4324}  & \multicolumn{1}{c}{5674}  & \multicolumn{1}{c|}{1245}        & 34101  & \multicolumn{1}{c}{107128}     & 41936   \\ 
% \textbf{Length} & \multicolumn{1}{c}{15.4}        & \multicolumn{1}{c}{6.4}    & \multicolumn{1}{c}{6.3}             & \multicolumn{1}{c}{8.1}   & \multicolumn{1}{c}{9.3}   & \multicolumn{1}{c|}{8.9}         & 6.5    & \multicolumn{1}{c}{1.0}        & 1.0     \\ \bottomrule
% \end{tabular}

% \caption{Basic statistics for navigation training data, comparing both our annotated dataset and different open-source data. Note that ``AC'' means Android Control dataset while the ``GUI-O'' represents GUI-Odyssey. We report the number of traces and their average lengths. The dataset marked with * means our collected.}
% \label{tab:navidata}
% \end{table*}

\begin{table*}[h]\small
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c|cccccc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Dataset}}           & \multicolumn{6}{c|}{\textbf{Multiple Steps}}                                                                                                                                                                         & \multicolumn{2}{c|}{\textbf{Single Step}}  & \multirow{2}{*}{\textbf{Sampled training set}}       \\ 
 & \multicolumn{1}{c}{{GUI-O}} & \multicolumn{1}{c}{{AITZ}} & \multicolumn{1}{c}{{AC}} & \multicolumn{1}{c}{{Aitw}}  & \multicolumn{1}{c}{{Amex}}  & \multicolumn{1}{c|}{{Navi*}}  & \multicolumn{1}{c}{{GD*}} & \multicolumn{1}{c|}{{VQA*}} &  \\ \hline
\textbf{\#Samples}     & \multicolumn{1}{c}{114k}      & \multicolumn{1}{c}{14k}  & \multicolumn{1}{c}{84k}           & \multicolumn{1}{c}{371k} & \multicolumn{1}{c}{39k} & \multicolumn{1}{c|}{20k}        & \multicolumn{1}{c}{107k}     & 42k & \textbf{350k}  \\ \
\textbf{\#Traces}    & \multicolumn{1}{c}{7k}        & \multicolumn{1}{c}{2k}   & \multicolumn{1}{c}{13k}           & \multicolumn{1}{c}{5k}  & \multicolumn{1}{c}{3k}  & \multicolumn{1}{c|}{*}          & \multicolumn{1}{c}{-}     & -  & * \\ \bottomrule
%\textbf{Length} & \multicolumn{1}{c}{15.4}        & \multicolumn{1}{c}{6.4}    & \multicolumn{1}{c}{6.3}             & \multicolumn{1}{c}{8.1}   & \multicolumn{1}{c}{9.3}   & \multicolumn{1}{c|}{8.9}         & 6.5    & \multicolumn{1}{c}{1.0}        & 1.0     \\ \bottomrule
\end{tabular}
\caption{Basic statistics for our collected navigation training data. Note that ``AC'' means Android Control dataset while the ``GUI-O'' represents GUI-Odyssey. The datasets marked with * means are collected by ourselves. Among these data, we select 350k high-quality samples as our training set.}
\label{tab:navidata}
\end{table*}


% multiple steps
% GUI-O：41300
% AITZ：10363 + 1647
% AITW：16410
% AC：42569
% Amex：34089
% Navi: 17685

% sinple steps
% GD：40000
% VQA：39006
% LOW：100000

==> tables/navi_online_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Qwen3-VL-2B~\citep{Qwen3-VL}                      &  2B    & 36.4                            \\ 
    Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    & 47.6                         \\ 
    Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &  54.3                       \\ 
    GLM-4.6V-Flash~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   9B        & 42.7  \\
    GLM-4.6V~\citep{vteam2025glm45vglm41vthinkingversatilemultimodal}       &   106B        & 57.0  \\
    Gemini-2.5-Pro~\citep{comanici2025gemini}  & -   &                    69.7      \\ 
    Seed1.8~\citep{seed1.8}  & -   &                    70.7      \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
    ScaleCUA-3B~\citep{}                      &  3B         & 23.7                           \\ 
    UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                      &  7B     & 30.0                     \\ 
    GUI-Owl-7B ~\citep{ye2025mobile}                      &  7B     &  66.4                    \\ 
    UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui}               &   72B    & 46.6  \\
    UI-Venus-1.0-7B~\citep{gu2025ui}                 &  7B & 49.1             \\ 
    UI-Venus-1.0-72B~\citep{gu2025ui}                &  72B     & 65.9               \\
    %OmegaUse-G~\citep{zhang2026omegausebuildinggeneralpurposegui} &  30B     &                \\
    Step-GUI-4B~\citep{yan2025step}  &  4B     & 63.9               \\ 
    Step-GUI-8B~\citep{yan2025step}                      &  8B     &                67.7      \\ 
    Holo2-8B~\citep{hai2025holo2modelfamily}                      &  8B     & 60.4                     \\ 
    Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                      &  30B     &  71.6                     \\ 
    MAI-UI-2B~\citep{zhou2025mai}                      &  2B     &    49.1                  \\ 
    MAI-UI-8B~\citep{zhou2025mai}                      &  8B     &  70.7                    \\ 
    MAI-UI-32B~\citep{zhou2025mai}                      &  32B     &  73.3                    \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &             \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{AndroidWorld} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:Androidworld}
\end{table}


==> tables/online_venus_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    &    6.7                      \\ 
    Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &  8.7                        \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\ 
    GUI-Owl-7B ~\citep{ye2025mobile}                      &  7B     &    6.7                  \\ 
    % MA3(GUI-Owl-7B)~\citep{ye2025mobile}                      &  7B     &                      \\ 
    UI-Venus-1.0-7B~\citep{gu2025ui}                &  7B &   8.1          \\ 
    UI-Venus-1.0-72B~\citep{gu2025ui}              &  72B &     15.4        \\ 
    Step-GUI-4B~\citep{yan2025step}  &  4B     &        8.0      \\ 
    MAI-UI-2B~\citep{zhou2025mai}                      &  2B     &                      \\ 
    MAI-UI-8B~\citep{zhou2025mai}                      &  8B     &     12.7                 \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &     16.1        \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &     21.5           \\ 
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{VenusBench-Mobile} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:VenusBench-Mobile}
\end{table}


==> tables/trainingdetails.tex <==
\begin{table}[ht]\small
\centering
% \footnotesize
\begin{tabular}{lccccc}
\toprule
    % save\_steps & 400 \\
\textbf{Hyperparameter} & \textbf{rollout} & \textbf{batch\_size} & \textbf{$\beta_{KL}$}  & \textbf{freeze\_vit} & \textbf{epoch}\\
\midrule
    \textbf{UI-Venus-Ground-7B}  & 8  & 128 & 4e-3 & False & 10  \\
    \textbf{UI-Venus-Ground-72B} & 10 & 128 & 4e-3 & False & 1  \\
    \textbf{UI-Venus-Navi-7B}    & 8  & 256 & 1e-3 & True  & 10  \\
   \textbf{UI-Venus-Navi-72B}    & 8  & 512 & 1e-3 & True  & 1 \\
\bottomrule
\end{tabular}
\vspace{0.4em}
\caption{Training hyperparameter settings used in the experiments of UI-Venus.}
\label{tab:hyper}
\end{table}

==> tables/webvoyager_exp.tex <==


\begin{table}[ht]
    \centering
    \footnotesize
    %\setlength{\tabcolsep}{0pt}
    \begin{tabular}{lcc}
    \toprule
    \textbf{Models} &\textbf{PARAS.}   & \textbf{Success Rate}                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{General VLMs}} \\
    Qwen3-VL-2B~\citep{Qwen3-VL}                      &  2B    &       35.21                     \\ 
    Qwen3-VL-8B ~\citep{Qwen3-VL}                      &  8B    &        45.26                  \\ 
    Qwen3-VL-30B-A3B ~\citep{Qwen3-VL}                      &  30B    &    47.55                      \\ 
    Gemini-2.5-Pro~\citep{comanici2025gemini}  & -   &                      \\ 
    Seed1.8~\citep{seed1.8}  & -   &                      \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{GUI-specific Models}} \\
    ScaleCUA-3B~\citep{}                      &  3B         &                           \\ 
    UI-TARS-1.5-7B~\citep{ui-tars-15-seed}                      &  7B     &                     \\ 
    GUI-Owl-7B ~\citep{}                      &  7B     &                      \\ 
    UI-TARS-72B~\citep{qin2025uitarspioneeringautomatedgui}               &   72B    &   \\
    Holo2-4B~\citep{hai2025holo2modelfamily}                      &  8B     &      80.2                \\ 
    Holo2-8B~\citep{hai2025holo2modelfamily}                     &  8B     &      80.2                \\ 
    Holo2-30B-A3B~\citep{hai2025holo2modelfamily}                   &  30B     &    83.0                  \\ 
    \midrule
    \rowcolor{gray!15}
    \multicolumn{3}{l}{\textit{Ours}} \\
    UI-Venus-1.5-2B              &  2B &             \\ 
    UI-Venus-1.5-8B              &  8B &             \\ 
    UI-Venus-1.5-30B-A3B              &  30B     &                \\ 
    
    \bottomrule
    \end{tabular}
    \vspace{0.4em}
    \caption{Performance comparison on \textbf{WebVoyager} for end-to-end models. Our UI-Venus-1.5 achieves state-of-the-art performance, outperforming all baseline methods across different settings.}
    \label{tab:webvoyager}
\end{table}

